Verified Self-Explaining Computation

Common programming tools, like compilers, debuggers, and IDEs, crucially rely on the ability to analyse program code to reason about its behaviour and properties. There has been a great deal of work on verifying compilers and static analyses, but far less on verifying dynamic analyses such as program slicing. Recently, a new mathematical framework for slicing was introduced in which forward and backward slicing are dual in the sense that they constitute a Galois connection. This paper formalises forward and backward dynamic slicing algorithms for a simple imperative programming language, and formally verifies their duality using the Coq proof assistant.

==> figs/liveness.tex <==
\begin{figure*}[t!]
 \begin{minipage}[b]{\textwidth}
  \small
  \begin{displaymath}
   \mathsf{live}(\skipKw, L) = L
   \ruleSpace
   \mathsf{live}(x := a, L) = \begin{cases}
     (L \setminus \{x\}) \cup \mathsf{fv}(a) & x \in L \\
     L & x \notin L \end{cases} % no blank line after this line!
   \ruleSpace
   \mathsf{live}(c_1\ ;;\ c_2, L) = \mathsf{live}(c_1, \mathsf{live}(c_2, L))
  \end{displaymath}

  \begin{displaymath}
    \mathsf{live}(\impIf, L) = \mathsf{fv}(b)\ \cup\ \mathsf{live}(c_1, L)\ \cup\ \mathsf{live}(c_2, L)
    \ruleSpace
    \mathsf{live}(\impWhile, L) = \mathsf{fix}\ (\lambda x.\ \mathsf{fv}(b)\ \cup\ L\ \cup\ \mathsf{live}(c, x))
  \end{displaymath}
 \end{minipage}

 %% \begin{tabular}{rcl}
 %%   $\mathsf{live}(L, \skipKw)$ & $=$ & $L$ \\
 %%   $\mathsf{live}(L, x := a)$      & $=$ & $\begin{cases}
 %%                                            (L \setminus \{x\})\ \cup\ \mathsf{fv}(a) & x \in L \\
 %%                                            L & x \notin L \end{cases}$ \\
 %%   $\mathsf{live}(L, c_1\ ;;\ c_2)$ & $=$ & $\mathsf{live}(\mathsf{live}(L, c_2), c_1)$ \\
 %%   $\mathsf{live}(L, \impIf)$ & $=$ & $\mathsf{fv}\ \cup\ \mathsf{live}(L, c_1)\ \cup\ \mathsf{live}(L, c_2)$ \\
 %%   $\mathsf{live}(L, \impWhile)$ & $=$ & $\mathsf{fix}(\lambda x.\ \mathsf{b}\ \cup\ L\ \cup\ \mathsf{live}(x, c))$ \\
 %% \end{tabular}

 \caption{Liveness analysis for Imp programs.}
 \label{fig:liveness}
\end{figure*}

